Accounting for News

Language-model embeddings of news explain returns but lack economic units. We define a text's meaning as the revision it induces in expected outcomes. An exact identity linking the outcomes divides the price move the text accounts for among fundamentals, later returns, and valuation. In a decade of 8-K filings, the text accounts for 5.5% of event-day return variance. Within a week, later returns add about a tenth to that part, mainly in smaller firms, and little to the remainder. That part carries 28% of the comovement between event-day returns and next-year sales growth, including sales from quarters begun after filing.

==> numbers.tex <==
\makeatletter
\@namedef{num@addB}{0.16}
\@namedef{num@addC}{0.41}
\@namedef{num@auAgeMed}{100}
\@namedef{num@auAgeNinety}{135}
\@namedef{num@auDaily}{15.8}
\@namedef{num@auDelW}{0.2}
\@namedef{num@auDelY}{6.4}
\@namedef{num@auFloor}{1}
\@namedef{num@auOnlyQ}{98.0}
\@namedef{num@auOtherAnn}{1.5}
\@namedef{num@bkAFm}{31}
\@namedef{num@bkAFy}{5}
\@namedef{num@bkAZm}{6.8}
\@namedef{num@bkAZy}{0.4}
\@namedef{num@cgAFm}{44}
\@namedef{num@cgAFq}{34}
\@namedef{num@cgAFy}{28}
\@namedef{num@cgAFyy}{17}
\@namedef{num@cgAZrm}{7.0}
\@namedef{num@cgAZrq}{5.9}
\@namedef{num@cgAZry}{5.9}
\@namedef{num@cgAZryy}{5.4}
\@namedef{num@chNoScG}{5.96}
\@namedef{num@chNoScGZ}{4.9}
\@namedef{num@chNoScWk}{\ensuremath{-}0.41}
\@namedef{num@chNoScWkZ}{\ensuremath{-}4.9}
\@namedef{num@ckTsew}{0.10}
\@namedef{num@ckTw}{0.56}
\@namedef{num@ckZAm}{2.7}
\@namedef{num@ckZAq}{1.7}
\@namedef{num@ckZAw}{5.8}
\@namedef{num@ckZabsw}{5.84}
\@namedef{num@cosBig}{\ensuremath{-}0.038}
\@namedef{num@cosBigZ}{1.2}
\@namedef{num@cosNoEaZ}{3.6}
\@namedef{num@cosSmall}{\ensuremath{-}0.154}
\@namedef{num@cosTw}{\ensuremath{-}0.119}
\@namedef{num@cosUw}{0.001}
\@namedef{num@ctsA}{4.7}
\@namedef{num@ctsB}{4.9}
\@namedef{num@ctsC}{5.1}
\@namedef{num@ctsD}{4.8}
\@namedef{num@cvNSATsey}{0.59}
\@namedef{num@cvNSATy}{3.67}
\@namedef{num@cvNSAZry}{5.2}
\@namedef{num@cvNSAZy}{5.20}
\@namedef{num@cvNSBTy}{\ensuremath{-}0.30}
\@namedef{num@desNoYesEarly}{3.4}
\@namedef{num@desYesYesEarly}{3.1}
\@namedef{num@dtNext}{1.8}
\@namedef{num@fielHi}{35}
\@namedef{num@fielLo}{23}
\@namedef{num@gAFm}{46}
\@namedef{num@gAFy}{28}
\@namedef{num@gAFyy}{15}
\@namedef{num@gATm}{1.85}
\@namedef{num@gATsm}{5.5}
\@namedef{num@gATy}{7.56}
\@namedef{num@gAWm}{3.99}
\@namedef{num@gAWry}{27}
\@namedef{num@gAWryy}{44}
\@namedef{num@gAWy}{26.53}
\@namedef{num@gAZbooty}{8.5}
\@namedef{num@gAZry}{8.0}
\@namedef{num@gEFm}{60}
\@namedef{num@gETy}{11.08}
\@namedef{num@gEZbootm}{7.6}
\@namedef{num@gEZrm}{9.8}
\@namedef{num@gNFy}{19}
\@namedef{num@gNFyy}{10}
\@namedef{num@gNTsy}{5.0}
\@namedef{num@gNZy}{3.67}
\@namedef{num@gNZyy}{1.64}
\@namedef{num@idB}{0.4}
\@namedef{num@idPost}{0.3}
\@namedef{num@idPre}{0.6}
\@namedef{num@idReg}{0.4}
\@namedef{num@idRegSE}{0.1}
\@namedef{num@kTsw}{5.3}
\@namedef{num@kTw}{0.61}
\@namedef{num@kWw}{0.77}
\@namedef{num@kZAm}{3.2}
\@namedef{num@kZAq}{3.4}
\@namedef{num@kZAw}{7.1}
\@namedef{num@kZabsw}{7.13}
\@namedef{num@kZbootw}{\ensuremath{-}7.1}
\@namedef{num@kZonew}{\ensuremath{-}7.1}
\@namedef{num@lgGapSeyyy}{0.61}
\@namedef{num@lgGapyyy}{0.27}
\@namedef{num@lgNoGapSeyyy}{0.36}
\@namedef{num@lgNoGapyyy}{\ensuremath{-}0.64}
\@namedef{num@lgRestY}{\ensuremath{-}0.24}
\@namedef{num@lgRestYY}{\ensuremath{-}0.42}
\@namedef{num@loqGHi}{7.77}
\@namedef{num@loqGLo}{7.23}
\@namedef{num@loqWkHi}{0.64}
\@namedef{num@loqWkLo}{0.58}
\@namedef{num@nA}{406,233}
\@namedef{num@nBook}{383,289}
\@namedef{num@nChronoWk}{374,354}
\@namedef{num@nFD}{406,000}
\@namedef{num@nFirms}{6,213}
\@namedef{num@nNoNews}{414,961}
\@namedef{num@nVS}{382,549}
\@namedef{num@nVSea}{108,723}
\@namedef{num@nVSfirms}{5,534}
\@namedef{num@nnGy}{22}
\@namedef{num@nnGyy}{39}
\@namedef{num@nnd}{4.6}
\@namedef{num@nnq}{8.3}
\@namedef{num@nnw}{7.3}
\@namedef{num@noItemShare}{1.1}
\@namedef{num@nofollowShare}{75}
\@namedef{num@oiAF}{33}
\@namedef{num@oiAT}{2.28}
\@namedef{num@oiAW}{6.91}
\@namedef{num@oiAZ}{6.6}
\@namedef{num@oiNT}{0.67}
\@namedef{num@oiNW}{2.50}
\@namedef{num@oiNZ}{3.0}
\@namedef{num@onB}{6.8}
\@namedef{num@onPost}{4.0}
\@namedef{num@onPre}{10.2}
\@namedef{num@onReg}{0.5}
\@namedef{num@onRegSE}{1.0}
\@namedef{num@osBig}{\ensuremath{-}0.047}
\@namedef{num@osBigZ}{1.8}
\@namedef{num@osEa}{\ensuremath{-}0.143}
\@namedef{num@osEaZ}{4.7}
\@namedef{num@osNoEa}{\ensuremath{-}0.093}
\@namedef{num@osNoEaZ}{5.5}
\@namedef{num@osNoFollow}{\ensuremath{-}0.129}
\@namedef{num@osPerA}{\ensuremath{-}0.105}
\@namedef{num@osPerB}{\ensuremath{-}0.110}
\@namedef{num@osPerC}{\ensuremath{-}0.121}
\@namedef{num@osPost}{\ensuremath{-}0.168}
\@namedef{num@osSmall}{\ensuremath{-}0.146}
\@namedef{num@osTd}{\ensuremath{-}0.059}
\@namedef{num@osTm}{\ensuremath{-}0.151}
\@namedef{num@osTq}{\ensuremath{-}0.308}
\@namedef{num@osTw}{\ensuremath{-}0.114}
\@namedef{num@osUd}{\ensuremath{-}0.004}
\@namedef{num@osUm}{\ensuremath{-}0.024}
\@namedef{num@osUq}{\ensuremath{-}0.058}
\@namedef{num@osUw}{\ensuremath{-}0.002}
\@namedef{num@osWLm}{\ensuremath{-}0.030}
\@namedef{num@osWLq}{\ensuremath{-}0.070}
\@namedef{num@osWLsew}{0.007}
\@namedef{num@osWLw}{\ensuremath{-}0.008}
\@namedef{num@osZd}{8.1}
\@namedef{num@osZw}{7.0}
\@namedef{num@payMax}{0.01}
\@namedef{num@plG}{\ensuremath{-}0.003}
\@namedef{num@plWk}{\ensuremath{-}0.002}
\@namedef{num@plWkZ}{2.2}
\@namedef{num@rAltChG}{9.82}
\@namedef{num@rAltChGZ}{2.8}
\@namedef{num@rAltChWk}{\ensuremath{-}0.29}
\@namedef{num@rAltChWkZ}{\ensuremath{-}2.1}
\@namedef{num@rAltG}{6.71}
\@namedef{num@rAltWk}{\ensuremath{-}0.44}
\@namedef{num@rChG}{7.94}
\@namedef{num@rChGZ}{5.9}
\@namedef{num@rChWk}{\ensuremath{-}0.56}
\@namedef{num@rChWkZ}{\ensuremath{-}5.8}
\@namedef{num@rNoGapG}{6.97}
\@namedef{num@rNoGapWk}{\ensuremath{-}0.61}
\@namedef{num@rNoGroupsG}{6.12}
\@namedef{num@rNoGroupsWk}{\ensuremath{-}0.47}
\@namedef{num@rRFG}{7.61}
\@namedef{num@rRFWk}{\ensuremath{-}0.62}
\@namedef{num@sLTw}{49}
\@namedef{num@sLTwt}{4.8}
\@namedef{num@sTm}{67}
\@namedef{num@sTw}{39}
\@namedef{num@sTwbig}{0}
\@namedef{num@sTwbigt}{0.0}
\@namedef{num@sTwea}{66}
\@namedef{num@sTweat}{4.5}
\@namedef{num@sTwmid}{30}
\@namedef{num@sTwmidt}{2.2}
\@namedef{num@sTwnoea}{18}
\@namedef{num@sTwnoeat}{1.3}
\@namedef{num@sTwsmall}{56}
\@namedef{num@sTwsmallt}{3.7}
\@namedef{num@sTwt}{3.5}
\@namedef{num@sUm}{51}
\@namedef{num@sUw}{14}
\@namedef{num@sUwea}{30}
\@namedef{num@sUweat}{2.5}
\@namedef{num@sUwsmall}{41}
\@namedef{num@sUwsmallt}{2.2}
\@namedef{num@sUwt}{1.3}
\@namedef{num@sWm}{71}
\@namedef{num@sWw}{29}
\@namedef{num@sWwsmall}{69}
\@namedef{num@tsAlt}{4.7}
\@namedef{num@tsB}{5.5}
\@namedef{num@tsBbig}{3.3}
\@namedef{num@tsBea}{5.7}
\@namedef{num@tsBgapY}{4.9}
\@namedef{num@tsBlate}{5.4}
\@namedef{num@tsBnoea}{5.3}
\@namedef{num@tsBnorel}{1.6}
\@namedef{num@tsBreg}{2.4}
\@namedef{num@tsBrel}{6.2}
\@namedef{num@tsBsmall}{5.8}
\@namedef{num@tsC}{4.7}
\@namedef{num@tsLead}{2.5}
\@namedef{num@tsNoGroups}{4.2}
\@namedef{num@tsPerm}{\ensuremath{-}0.001}
\@namedef{num@tsPermSE}{0.002}
\@namedef{num@tsRF}{5.6}
\@namedef{num@tsRaw}{4.6}
\@namedef{num@tsTitle}{1.7}
\@namedef{num@tsTyAgree}{11.7}
\@namedef{num@tsTyEarn}{6.1}
\@namedef{num@tsTyOther}{6.0}
\@namedef{num@vESAFy}{34}
\@namedef{num@vESATsey}{0.75}
\@namedef{num@vESATy}{4.60}
\@namedef{num@vESEFy}{71}
\@namedef{num@vESETy}{4.77}
\@namedef{num@vESPFy}{47}
\@namedef{num@vESPTy}{3.30}
\@namedef{num@vNNSTsey}{0.49}
\@namedef{num@vNNSTy}{\ensuremath{-}1.04}
\@namedef{num@vNSAFy}{34}
\@namedef{num@vNSATy}{3.58}
\@namedef{num@vNSATyy}{4.47}
\@namedef{num@vNSAWy}{10.49}
\@namedef{num@vNSAWyy}{19.27}
\@namedef{num@vNSAZry}{4.7}
\@namedef{num@vNSAZy}{4.73}
\@namedef{num@vNSAZyy}{3.47}
\@namedef{num@vNSBTsey}{0.22}
\@namedef{num@vNSBTy}{\ensuremath{-}0.29}
\@namedef{num@vNSPTy}{2.20}
\@namedef{num@vNSPWy}{4.25}
\@namedef{num@vsTm}{0.83}
\@namedef{num@vsTq}{0.85}
\@namedef{num@vsUm}{1.01}
\@namedef{num@vsUq}{1.01}
\@namedef{num@vsZm}{3.3}
\@namedef{num@vsZq}{1.4}
\@namedef{num@wG}{7.13}
\@namedef{num@wGRaw}{7.58}
\@namedef{num@wWk}{\ensuremath{-}0.58}
\@namedef{num@wWkRaw}{\ensuremath{-}0.60}
\@namedef{num@yrsG}{10 of 10}
\@namedef{num@yrsWk}{9 of 10}
\@namedef{num@zmaxA}{8.0}
\@namedef{num@zminA}{3.7}
\makeatother

